Type Theory as a Language Workbench

Language Workbenches offer language designers an expressive environment in which to create their DSLs. Similarly, research into mechanised meta-theory has shown how dependently typed languages provide expressive environments to formalise and study DSLs and their meta-theoretical properties. But can we claim that dependently typed languages qualify as language workbenches? We argue yes! We have developed an exemplar DSL called Velo that showcases not only dependently typed techniques to realise and manipulate IRs, but that dependently typed languages make fine language workbenches. Velo is a simple verified language with well-typed holes and comes with a complete compiler pipeline: parser, elaborator, REPL, evaluator, and compiler passes. Specifically, we describe our design choices for well-typed IRs design that includes support for well-typed holes, how CSE is achieved in a well-typed setting, and how the mechanised type-soundness proof for Velo is the source of the evaluator.

==> Code/MiniCompact.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Code.MiniCompact}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Code.MiniVelo}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Code.MiniDeBruijn}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}


%<*PrimDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Prim}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{args}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisType{Ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ret}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Zero}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Prim}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{TyNat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Inc}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Prim}\KatlaSpace{}\IdrisData{[TyNat]}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{TyNat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{App}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Prim}\KatlaSpace{}\IdrisData{[TyArr}\KatlaSpace{}\IdrisBound{dom}\KatlaSpace{}\IdrisBound{cod}\IdrisData{,}\KatlaSpace{}\IdrisBound{dom}\IdrisData{]}\KatlaSpace{}\IdrisBound{cod}\KatlaNewline{}
\end{code}
%</PrimDef>

\begin{code}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Terms}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ctxt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisType{Ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisType{Ty}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\end{code}


\begin{code}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*TermDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ctxt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisType{Ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Ty}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Var}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{IsVar}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{ty}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{ty}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Fun}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ctxt}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{TyArr}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Call}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{tys}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{operator}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Prim}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{tys}\KatlaSpace{}\KatlaSpace{}\IdrisBound{ty}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{operands}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Terms}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{tys}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{ty}\KatlaNewline{}
\end{code}
%</TermDef>

\begin{code}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*AllDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Terms}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ctxt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisType{Ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisType{Ty}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Nil}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Terms}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisData{Nil}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{(::)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{ty}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Terms}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{tys}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Terms}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ty}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{tys}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</AllDef>



==> Code/MiniDeBruijn.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Code.MiniDeBruijn}\KatlaNewline{}
\end{code}

%<*AtIndexDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{AtIndex}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ty}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{kind}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ctxt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{kind}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{idx}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Here}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{AtIndex}\KatlaSpace{}\IdrisBound{ty}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ctxt}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{There}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{AtIndex}\KatlaSpace{}\IdrisBound{ty}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{idx}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{AtIndex}\KatlaSpace{}\IdrisBound{ty}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ctxt}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{1}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{idx}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</AtIndexDef>

\begin{code}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*IsVarDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{IsVar}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ctxt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{kind}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ty}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{kind}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{V}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{idx}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{prf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{AtIndex}\KatlaSpace{}\IdrisBound{ty}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{idx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IsVar}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{ty}\KatlaNewline{}
\end{code}
%</IsVarDef>



==> Code/MiniExecute.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Code.MiniExecute}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Code.MiniVelo}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Code.MiniCompact}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%hide}\KatlaSpace{}MiniVelo.Term\KatlaNewline{}
\KatlaNewline{}
\IdrisFunction{subst}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ctxt}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Value}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{ty}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\end{code}

\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Reduxes}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{these}\IdrisKeyword{,}\IdrisBound{those}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Terms}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{tys}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\end{code}

%<*ReduxDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Redux}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{this}\IdrisKeyword{,}\IdrisBound{that}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{SimplifyCall}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{op}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Prim}\KatlaSpace{}\IdrisBound{tys}\KatlaSpace{}\IdrisBound{ty}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{step}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Reduxes}\KatlaSpace{}\IdrisBound{these}\KatlaSpace{}\IdrisBound{those}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Redux}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Call}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{these}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Call}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{those}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{ReduceFuncApp}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{body}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ctxt}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{type}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{return}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{arg}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{type}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{value}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Value}\KatlaSpace{}\IdrisBound{arg}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Redux}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Call}\KatlaSpace{}\IdrisData{App}\KatlaSpace{}\IdrisData{[Fun}\KatlaSpace{}\IdrisBound{body}\IdrisData{,}\KatlaSpace{}\IdrisBound{arg}\IdrisData{]}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{subst}\KatlaSpace{}\IdrisBound{arg}\KatlaSpace{}\IdrisBound{body}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</ReduxDef>

%<*ReducesDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Reduxes}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{these}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{those}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Terms}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{tys}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{(!:)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{hd}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Redux}\KatlaSpace{}\IdrisBound{this}\KatlaSpace{}\IdrisBound{that}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{rest}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Terms}\KatlaSpace{}\IdrisBound{ctxt}\KatlaSpace{}\IdrisBound{tys}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Reduxes}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{this}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{rest}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{that}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{rest}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{(::)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{value}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Value}\KatlaSpace{}\IdrisBound{hd}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{tl}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Reduxes}\KatlaSpace{}\IdrisBound{these}\KatlaSpace{}\IdrisBound{those}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Reduxes}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{these}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{those}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</ReducesDef>

\begin{code}
\IdrisFunction{Pred}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\IdrisFunction{Pred}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaNewline{}
\IdrisFunction{Rel}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\IdrisFunction{Rel}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Pred}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\end{code}

%<*ProgressDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Progress}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{value}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Pred}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{redux}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Rel}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{tm}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{where}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{tm}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{val}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{value}\KatlaSpace{}\IdrisBound{tm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Progress}\KatlaSpace{}\IdrisBound{value}\KatlaSpace{}\IdrisBound{redux}\KatlaSpace{}\IdrisBound{tm}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Step}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{this}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{that}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{step}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{redux}\KatlaSpace{}\IdrisBound{this}\KatlaSpace{}\IdrisBound{that}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Progress}\KatlaSpace{}\IdrisBound{value}\KatlaSpace{}\IdrisBound{redux}\KatlaSpace{}\IdrisBound{this}\KatlaNewline{}
\end{code}
%</ProgressDef>

\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{RTList}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Rel}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Rel}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\end{code}

%<*ResultDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Result}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{value}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Pred}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{redux}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Rel}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{this}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{where}\KatlaSpace{}\IdrisData{R}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{that}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{val}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{value}\KatlaSpace{}\IdrisBound{that}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{steps}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{RTList}\KatlaSpace{}\IdrisBound{redux}\KatlaSpace{}\IdrisBound{this}\KatlaSpace{}\IdrisBound{that}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Result}\KatlaSpace{}\IdrisBound{value}\KatlaSpace{}\IdrisBound{redux}\KatlaSpace{}\IdrisBound{this}\KatlaNewline{}
\end{code}
%</ResultDef>



==> Code/MiniVelo.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Code.MiniVelo}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}

%<*TyDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Ty}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{TyNat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{TyBool}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{TyArr}\KatlaSpace{}\IdrisType{Ty}\KatlaSpace{}\IdrisType{Ty}\KatlaNewline{}
\end{code}
%</TyDef>

\begin{code}
\IdrisKeyword{\%hide}\KatlaSpace{}Prelude.SnocList\KatlaNewline{}
\end{code}

%<*SnocListDef>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Lin}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{(:<)}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\end{code}
%</SnocListDef>

%<*ElemTermDecl>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Elem}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{gamma}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{gamma}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisType{Ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\end{code}
%</ElemTermDecl>

%<*ElemDecl>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Elem}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{gamma}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\end{code}
%</ElemDecl>
\begin{code}
\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\end{code}
%<*varZero>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Here}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Elem}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{gamma}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{ty}\KatlaNewline{}
\end{code}
%</varZero>

\end{code}
%<*varSuc>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisData{There}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\KatlaSpace{}\IdrisType{Elem}\KatlaSpace{}\IdrisBound{gamma}\KatlaSpace{}\IdrisBound{ty}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Elem}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{gamma}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisBound{ty}\KatlaNewline{}
\end{code}
%</varSuc>

\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{gamma}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisType{Ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{type}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\end{code}

%<*inferenceZero>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Zero}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{gamma}\KatlaSpace{}\IdrisData{TyNat}\KatlaNewline{}
\end{code}
%</inferenceZero>


%<*inferenceVar>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Var}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\KatlaSpace{}\IdrisType{Elem}\KatlaSpace{}\IdrisBound{gamma}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{gamma}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\end{code}
%</inferenceVar>


%<*inferenceInc>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Inc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{gamma}\KatlaSpace{}\IdrisData{TyNat}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{gamma}\KatlaSpace{}\IdrisData{TyNat}\KatlaNewline{}
\end{code}
%</inferenceInc>


%<*inferenceApp>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisData{App}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{gamma}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{TyArr}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{gamma}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{gamma}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\end{code}
%</inferenceApp>


%<*inferenceFunc>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Func}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{gamma}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisBound{gamma}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{TyArr}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</inferenceFunc>


%<*Plus2Def>
\begin{code}
\IdrisFunction{Plus2}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{TyArr}\KatlaSpace{}\IdrisData{TyNat}\KatlaSpace{}\IdrisData{TyNat}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{Plus2}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Func}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Inc}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Inc}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Var}\KatlaSpace{}\IdrisData{Here}\IdrisKeyword{)))}\KatlaNewline{}
\end{code}
%</Plus2Def>

%<*IllScoped>
\begin{code}
\IdrisKeyword{failing}\KatlaSpace{}\IdrisData{"Mismatch\KatlaSpace{}between:\KatlaSpace{}?gamma\KatlaSpace{}:<\KatlaSpace{}TyNat\KatlaSpace{}and\KatlaSpace{}[<]."}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Ouch}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisData{TyNat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Ouch}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Var}\KatlaSpace{}\IdrisData{Here}\KatlaNewline{}
\end{code}
%</IllScoped>

%<*IllTyped>
\begin{code}
\IdrisKeyword{failing}\KatlaSpace{}\IdrisData{"Mismatch\KatlaSpace{}between:\KatlaSpace{}TyBool\KatlaSpace{}and\KatlaSpace{}TyNat."}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Ouch}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Term}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{TyArr}\KatlaSpace{}\IdrisData{TyNat}\KatlaSpace{}\IdrisData{TyBool}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Ouch}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Func}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Var}\KatlaSpace{}\IdrisData{Here}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</IllTyped>



==> content/efficientdeceq.tex <==
\subsection{Efficient Decidable Equality}
\label{sec:idioms:decEq}

Users do not always have access to a meta-program that supports the deriving of a proof that propositional equality is decidable for their data structures~\cite{DBLP:conf/icfp/ChristiansenB16}.
%
In such cases, the most common strategy is to use nested pattern matching and produce
clauses quadratic in the number of constructors for the specified data structure.
%
Na{\"i}vely one can reduce the number of contradictions to prove using symmetry breaking (\IdrisFunction{negEqSym}), but the number of cases to present is still many.
%
We can, however, reduce the complexity of \IdrisType{DecEq} instance creation from quadratic to linear in the number of constructors.
%

For example, consider the following standard definition of a binary tree:

\begin{Verbatim}
data Bin = Leaf | Node Bin Bin
\end{Verbatim}

\noindent
We first define a diagonal relation (\IdrisType{Diag}) that requires that two terms must have the same top-level constructor.

\begin{Verbatim}
data Diag : (s, t : Bin) -> Type where
  Leaf2 : Diag Leaf Leaf
  Node2 : (s, t, u, v : Bin) -> Diag (Node s t) (Node u v)
\end{Verbatim}

\noindent
Using \IdrisType{Diag} we can define a function, \IdrisFunction{diag}, function that, from two terms, either returns a proof that they satisfy the \IdrisType{Diag} relation or return \IdrisData{Nothing}.

\begin{Verbatim}
diag : (s, t : Bin) -> Maybe (Diag s t)
diag Leaf       Leaf       = Just Leaf2
diag (Node s t) (Node u v) = Just (Node2 s t u v)
diag _          _          = Nothing
\end{Verbatim}

\noindent
We can easily prove that \IdrisFunction{diag} cannot possibly return \IdrisData{Nothing} if the inputs are in fact equal.

\begin{Verbatim}
diagNot : (t : Bin) -> Not (diag t t === Nothing)
diagNot Leaf       = absurd
diagNot (Node _ _) = absurd
\end{Verbatim}

\noindent
We can use \IdrisFunction{diagNot} to implement \IdrisFunction{decEq}
by only considering cases where the two input terms share the same
top-level constructor.
For the remaining cases we only require a generic catch-all case that handles all top-level mismatches thanks to \IdrisFunction{diagNot}.

\begin{Verbatim}
decEq : (s, t : Bin) -> Dec (s === t)
decEq s@_ t@_ with (diag s t) proof eq
  _ | Just Leaf2 = Yes Refl
  _ | Just (Node2 a b u v) with (decEq a u) | (decEq b v)
    _ | Yes eq1 | Yes eq2 = Yes (cong2 Node eq1 eq2)
    _ | No neq1 | _ = No (\textbackslash{}case Refl => neq1 Refl)
    _ | _ | No neq2 = No (\textbackslash{}case Refl => neq2 Refl)
  _ | Nothing = No (\textbackslash{} Refl => diagNot _ eq)
\end{Verbatim}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> content/positivelynegative.tex <==
\subsection{Being Positively Negative}
\label{sec:idioms:posneg}

A workhorse of dependently typed programming is using decidable
predicates that capture, and produce, positive information.
We can represent the results of a decidable function using \texttt{Dec}:

\begin{Verbatim}
data Dec a = Yes a | No (a -> Void)
\end{Verbatim}

\noindent
Notice that in the negative position (the \texttt{No} constructor) we do not return positive information.
We provide a proof of falsity.
When reasoning about our programs such proof of falsity is good.
When interacting with our programs such proof of falsity is not good.
Consider the following type signatures that specify two decidable procedures.
The first to determine if one natural number is greater than another.

\begin{Verbatim}
isGT : (x,y : Nat) -> Dec (GT x y)
\end{Verbatim}

\noindent
The other, \IdrisFunction{any}, determines if any element in the list satisfies a supplied predicate.

\begin{Verbatim}
any : (f  : (x : type) -> Dec (p x)) -> (xs : List type) -> Dec (Any p xs)
\end{Verbatim}

For \IdrisFunction{isGT} we know that if the result is negative we can safely assume that \IdrisType{GT} \IdrisImplicit{x y} is false.
With \IdrisFunction{any} we do not know for sure why the decidable procedure failed.
Was it because the list was empty?
or,
was it because all elements of \IdrisBound{xs} did not satisfy \IdrisImplicit{p}!?
Furthermore, we cannot programmatically determine the reason why an element in \IdrisBound{xs} did not satisfy \IdrisImplicit{p}?

To address these issues. we introduce \IdrisType{DecInfo} a variant of \IdrisType{Dec} that carries positive information in the negative case, as well as proofs-of-falsity.

\chcomment[id=gallais]
          {Do we want to spend precious space talking about DecInfo
            rather than going straight to the nicest solution?}
\chcomment[id=jfdm]
          {But we do not use the nicest solution...}

\begin{Verbatim}
data DecInfo e p = Yes p | No e (p -> Void)
\end{Verbatim}

With this simple change we can now report \emph{why} a decision procedure failed, as well as proof that it failed.
Our examples can now become:

\begin{Verbatim}
isGT : (x,y : Nat) -> DecInfo (LTE x y) (GT x y)
\end{Verbatim}

\noindent
and

\begin{Verbatim}
any : (f  : (x : type) -> Dec (q x) (p x))
   -> (xs : List type)
         -> DecInfo (All (\textbackslash{}x => Pair (q x) (Not (p x))) xs) (Any p xs)
\end{Verbatim}

\IdrisType{DecInfo} does, however, carry a proof of false.
A more interesting line of work would be to adopt \emph{constructive negation} to ensure that proofs of false arise from positive sources only~\cite{msfp/Atkey22}.
That is, given:

\begin{Verbatim}
Predicate : Type
Predicate = (pos ** neg ** (pos -> neg -> Void))
\end{Verbatim}

\noindent
we can recreate \IdrisType{DecInfo} as:

\begin{Verbatim}
DecInfo : Predicate -> Type
DecInfo (pos ** neg ** no) = Either neg pos
\end{Verbatim}

\noindent
Being \emph{positively negative} stems back to producing good error messages when implementing elaborators~\cite{DBLP:journals/jfp/McBrideM04}.
We are investigating the efficacy of being \emph{positively negative} and how that impacts program design in dependently typed languages.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> figure/dynamics-smallstep.tex <==
\begin{mathpar}%\mprset{sep=1em}
  %
  % Naturals
  %
  \and
  \infer*[left=Z-Val]
  {%
    \\
  }{%
    \exprZero{}\StepTo\exprZero{}
  }
  \and
  \infer*[left=Inc]
  {%
    n\StepsTo{v}
  }{%
    \exprIncRule\StepsTo{\exprIncValue}
  }
  \and
  \infer*[left=Add-L]
  {%
    a\StepsTo{v}
  }{%
    \exprAddRule\StepsTo{\exprAddStepL}
  }
  \and
  \infer*[left=Add-LZ]
  {%
    b\StepsTo{v}
  }{%
    \exprAddValueLZ\StepsTo{v}
  }
  \and
  \infer*[left=Add-RV]
  {%
    b\StepsTo{v_b}
  }{%
    \exprAddValueRV\StepsTo{\exprAddStepValue}
  }
  %
  % Booleans
  %
  \and
  \infer*[left=T-Val]
  {%
    \\
  }{%
    \exprTrue\StepTo\exprTrue
  }
  \and
  \infer*[left=F-Val]
  {%
    \\
  }{%
    \exprFalse\StepTo\exprFalse
  }
  \and
  \infer*[left=And-L]
  {%
    a\StepsTo{v}
  }{%
    \exprAndRule\StepsTo{\exprAndStepL}
  }
  \and
  \infer*[left=And-TR]
  {%
    b\StepsTo{v}
  }{%
    \exprAndValueL\StepsTo{v}
  }
  \and
  \infer*[left=And-FW]
  {%
    \\
  }{%
    \exprAndValueF\StepsTo{\exprFalse}
  }
  \and
  \infer*[left=App]
  {%
    f\StepsTo{\exprLamValue}
  }{%
    \exprAppRule\StepsTo\subst{b}{x}{a}
  }
\end{mathpar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> figure/statics.tex <==
\begin{mathpar}%\mprset{sep=1em}
  \infer*[left=Var]
  {%
    \ty{x}{t}\in\Gamma
  }{%
    \env{\ty{x}{t}}
  }
  %
  % Naturals
  %
  \and
  \infer*[left=Z-Intro]
  {%
    \\
  }{%
    \env{\ty{\exprZero}{\TyNat}}
  }
  \and
  \infer*[left=Inc]
  {%
    \env{\ty{n}{\TyNat}}
  }{%
    \env{\ty{\exprIncRule}{\TyNat}}
  }
  \and
  \infer*[left=Add]
  {%
    \env{\ty{a}{\TyNat}}
    \\
    \env{\ty{b}{\TyNat}}
  }{%
    \env{\ty{\exprAddRule}{\TyNat}}
  }
  %
  % Booleans
  %
  \and
  \infer*[left=T-Intro]
  {%
    \\
  }{%
    \env{\ty{\exprTrue}{\TyBool}}
  }
  \and
  \infer*[left=F-Intro]
  {%
    \\
  }{%
    \env{\ty{\exprFalse}{\TyBool}}
  }
  \and
  \infer*[left=And]
  {%
    \env{\ty{a}{\TyBool}}
    \\
    \env{\ty{b}{\TyBool}}
  }{%
    \env{\ty{\exprAndRule}{\TyBool}}
  }
  %
  % Lam & Apps
  %
  \and
  \infer*[left=Lam]
  {%
    \env[\envAdd{\ty{x}{t_a}}]{\ty{b}{t_b}}
  }{%
    \env{\ty{\exprLamRule}{\typeFuncRule}}
  }
  \and
  \infer*[left=App]
  {%
    \env{\ty{f}{\typeFuncRule}}
    \\
    \env{\ty{a}{t_a}}
  }{%
    \env{\ty{\exprAppRule}{t_b}}
  }
  %
  % Lets
  %
  \and
  \infer*[left=Let]
  {%
    \env{\ty{e}{t_a}}
    \\
    \env[\envAdd{\ty{x}{t_a}}]{\ty{b}{t_b}}
  }{%
    \env{\ty{\exprLetRule}{t_b}}
  }
\end{mathpar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> notations.tex <==
%% Temporary shim before we bring in Katla's idris2.sty

\newcommand{\IdrisData}[1]{\texttt{#1}}
\newcommand{\IdrisType}[1]{\texttt{#1}}
\newcommand{\IdrisFunction}[1]{\texttt{#1}}
\newcommand{\IdrisImplicit}[1]{\texttt{#1}}
\newcommand{\IdrisBound}[1]{\texttt{#1}}


==> robust-catch.tex <==
\makeatletter

\newrobustcmd*\OrigExecuteMetaData[2][\jobname]{%
\CatchFileBetweenTags\CatchFBT@tok{#1}{#2}%
\global\expandafter\CatchFBT@tok\expandafter{%
\expandafter}\the\CatchFBT@tok
}%\OrigExecuteMetaData

\newrobustcmd*\ChkExecuteMetaData[2][\jobname]{%
\CatchFileBetweenTags\CatchFBT@tok{#1}{#2}%
\edef\mytokens{\detokenize\expandafter{\the\CatchFBT@tok}}
\ifx\mytokens\empty\PackageError{catchfilebetweentags}{the tag #2 is not found\MessageBreak in file #1 \MessageBreak called from \jobname.tex}{use a different tag}\fi%
}%\ChkExecuteMetaData

\renewrobustcmd*\ExecuteMetaData[2][\jobname]{%
\ChkExecuteMetaData[#1]{#2}%
\OrigExecuteMetaData[#1]{#2}%
}

\makeatother

